Making Progress Based on False Discoveries

The study of adaptive data analysis examines how many statistical queries can be answered accurately using a fixed dataset while avoiding false discoveries (statistically inaccurate answers). In this paper, we tackle a question that precedes the field of study: Is data only valuable when it provides accurate answers to statistical queries? To answer this question, we use Stochastic Convex Optimization as a case study. In this model, algorithms are considered as analysts who query an estimate of the gradient of a noisy function at each iteration and move towards its minimizer. It is known that $O(1/\epsilon^2)$ examples can be used to minimize the objective function, but none of the existing methods depend on the accuracy of the estimated gradients along the trajectory. Therefore, we ask: How many samples are needed to minimize a noisy convex function if we require $\epsilon$-accurate estimates of $O(1/\epsilon^2)$ gradients? Or, might it be that inaccurate gradient estimates are \emph{necessary} for finding the minimum of a stochastic convex function at an optimal statistical rate? We provide two partial answers to this question. First, we show that a general analyst (queries that may be maliciously chosen) requires $\Omega(1/\epsilon^3)$ samples, ruling out the possibility of a foolproof mechanism. Second, we show that, under certain assumptions on the oracle, $\tilde \Omega(1/\epsilon^{2.5})$ samples are necessary for gradient descent to interact with the oracle. Our results are in contrast to classical bounds that show that $O(1/\epsilon^2)$ samples can optimize the population risk to an accuracy of $O(\epsilon)$, but with spurious gradients.

==> header_colt.tex <==
\usepackage[utf8]{inputenc}



\usepackage{mathtools}
\usepackage[capitalise]{cleveref}

%%commands the interfere with colt
%\usepackage{amsmath,amsfonts,amsthm,amssymb}
%\usepackage[margin=1in]{geometry}
%\usepackage[capitalise]{cleveref}

%% \declaretheorem[parent=section]{theorem}
%\declaretheorem[parent=section]{theorem}
%\declaretheorem[parent=section]{lemma}
%\declaretheorem[sibling=theorem]{corollary}
%\declaretheorem{claim}
%\declaretheorem{observation}
%\declaretheorem[parent=section]{definition}
%\declaretheorem{remark}
%\newtheorem*{theorem*}{Theorem}
%\newtheorem{proposition}{Proposition}
%\let\proof\undefined
%\declaretheoremstyle[
%        spaceabove=\topsep, 
%        spacebelow=\topsep, 
%        % headfont=\normalfont\bfseries,
%        bodyfont=\normalfont,
%        notefont=\normalfont\bfseries,
%        % notebraces={(}{)},
%        notebraces={}{},
%        % postheadspace=0.33em, 
%        qed=$\blacksquare$, 
%        % headpunct={},
%        % postfoothook=\noindent\ignorespaces
%    ]{proofstyle}
%\declaretheorem[style=proofstyle,numbered=no,name=Proof]{proof}
% \usepackage[hidelinks,colorlinks=true,linkcolor=blue,citecolor=blue]{hyperref}
%\crefname{claim}{Claim}{Claims}


\newtheorem*{theorem*}{Theorem}

% Times
% \usepackage{mytimes}

% New Century Schoolbook
% \usepackage{scholax}
% % \usepackage{tgschola}
% \usepackage[scaled=1.0,ncf,vvarbb]{newtxmath}
\usepackage[numbers]{natbib} 
\usepackage{thmtools,thm-restate}


\usepackage{xcolor}
\usepackage[extdef=true]{delimset}
\usepackage{xspace}
\usepackage{crossreftools}

\pdfstringdefDisableCommands{%
    \let\Cref\crtCref
    \let\cref\crtcref
}





% \usepackage[todonotes={textsize=footnotesize}]{changes}
% % \usepackage[final]{changes}
% \definechangesauthor[name=TK]{TK}
% \definechangesauthor[name=RL,color=magenta]{RL}
% \definechangesauthor[name=IA,color=teal]{IA}



% some defs
\newcommand{\reals}{\mathbb{R}}
\newcommand{\spn}{\mathrm{span}}
\DeclareMathOperator*{\spnb}{span^{\mathcal{B}_r}}
\DeclareMathOperator*{\spnone}{span^{1}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\E}{\mathop{\mathbb{E}}}
\newcommand{\dotp}{\boldsymbol{\cdot}}
\newcommand{\hsep}{\vspace{2ex}\noindent\rule{\textwidth}{1pt}\vspace{2ex}}
\DeclareMathOperator*{\argmax}{\arg\max}
\DeclareMathOperator*{\argmin}{\arg\min}
\DeclareMathOperator*{\sign}{sign}
\DeclareMathOperator*{\rem}{remainder}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\bigceil{\Big\lceil}{\Big\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\bigfloor{\Big\lfloor}{\Big\rfloor}
\newcommand{\wrgd}{w^{\lambda\textrm{GD}}}
\newcommand{\wgd}{w^{\textrm{GD}}}
\newcommand{\wsgd}{w^{\textrm{SGD}}}
\newcommand{\etabar}{\overline\eta}
\newcommand{\wbar}{\overline{w}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\betabar}{\bar{\beta}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cI}{\mathcal{I}(S)}
\newcommand{\cIt}[1]{\mathcal{I}_{#1}(S)}
\newcommand{\cIminus}{\mathcal{I}^-}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\f}[1]{f_{\scriptscriptstyle {(#1)}}}
\newcommand{\F}[1]{F_{\scriptscriptstyle {(#1)}}}
\newcommand{\medcup}{\textstyle \bigcup}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\epsilonbold}{\boldsymbol{\epsilon}}

\newcommand{\discolorlinks}[1]{{\hypersetup{hidelinks}#1}}

\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\ignore}[1]{}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\construct}[1]{\f{\discolorlinks{\ref{#1}}}}
\newcommand{\ffull}{\construct{eq:construction}}
\newcommand{\fsimple}{\construct{eq:construction_simple}}

% \newcommand{\fsimple}{\f{\discolorlinks{\ref{eq:construction_simple}}}}

\newcommand{\grad}{\nabla}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\rd}{\reals^d}
\newcommand{\V}{E}
\renewcommand{\Z}{\mathcal{Z}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\B}{\mathcal{B}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\lkana}{(\ell,k)\textrm{-analyst}}
\newcommand{\q}{\mathbf{q}}
\renewcommand{\a}{\mathbf{a}}
\renewcommand{\b}{\mathbf{b}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\fa}{f^{(A)}}
\newcommand{\sib}{\textrm{sib}}
\newcommand{\son}{\textrm{dec}}
\newcommand{\fat}{\textrm{pred}}
\newcommand{\state}{s}
\newcommand{\State}{\mathcal{S(A)}}
\newcommand{\depth}{d}
\renewcommand{\root}{e_r}
\newcommand{\T}{\mathcal{T}}
\renewcommand{\N}{\mathcal{N}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\fla}{FOA\xspace}
